3D Inception-based CNN with sMRI and MD-DTI data fusion for Alzheimer's Disease diagnostics

In the last decade, computer-aided early diagnostics of Alzheimer's Disease (AD) and its prodromal form, Mild Cognitive Impairment (MCI), has been the subject of extensive research. Some recent studies have shown promising results in the AD and MCI determination using structural and functional Magnetic Resonance Imaging (sMRI, fMRI), Positron Emission Tomography (PET) and Diffusion Tensor Imaging (DTI) modalities. Furthermore, fusion of imaging modalities in a supervised machine learning framework has shown promising direction of research. In this paper we first review major trends in automatic classification methods such as feature extraction based methods as well as deep learning approaches in medical image analysis applied to the field of Alzheimer's Disease diagnostics. Then we propose our own design of a 3D Inception-based Convolutional Neural Network (CNN) for Alzheimer's Disease diagnostics. The network is designed with an emphasis on the interior resource utilization and uses sMRI and DTI modalities fusion on hippocampal ROI. The comparison with the conventional AlexNet-based network using data from the Alzheimer's Disease Neuroimaging Initiative (ADNI) dataset (http://adni.loni.usc.edu) demonstrates significantly better performance of the proposed 3D Inception-based CNN.

==> architectures.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccc}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}configuration\\ name\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}number of\\ convolutional\\ layers\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}convolution kernel\\ size for each layer\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}number of\\ convolutional filters\\ in each layer\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}number of\\ fully-connected\\ layers\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}number of units in\\  each fully-connected\\  layer\end{tabular}} \\ \hline
C1 & 4 & (5, 4, 3, 3) & (16, 32, 64, 128) & 2 & (16, 8) \\
C2 & 5 & (5, 4, 3, 3, 3) & (16, 32, 64, 128, 128) & 2 & (16, 8) \\
C3 & 5 & (7, 6, 5, 4, 3) & (16, 32, 64, 128, 256) & 2 & (32, 8) \\
C4 & 6 & (7, 6, 5, 4, 3, 3) & (16, 32, 64, 128, 256, 256) & 1 & 16 \\ \hline
\end{tabular}%
}
\caption{Compared architectures of the used neural networks}
\label{table:architectures}
\end{table*}

